Look, Listen, and Attack: Backdoor Attacks Against Video Action Recognition

Deep neural networks (DNNs) are vulnerable to a class of attacks called "backdoor attacks", which create an association between a backdoor trigger and a target label the attacker is interested in exploiting. A backdoored DNN performs well on clean test images, yet persistently predicts an attacker-defined label for any sample in the presence of the backdoor trigger. Although backdoor attacks have been extensively studied in the image domain, there are very few works that explore such attacks in the video domain, and they tend to conclude that image backdoor attacks are less effective in the video domain. In this work, we revisit the traditional backdoor threat model and incorporate additional video-related aspects to that model. We show that poisoned-label image backdoor attacks could be extended temporally in two ways, statically and dynamically, leading to highly effective attacks in the video domain. In addition, we explore natural video backdoors to highlight the seriousness of this vulnerability in the video domain. And, for the first time, we study multi-modal (audiovisual) backdoor attacks against video action recognition models, where we show that attacking a single modality is enough for achieving a high attack success rate.

==> sections/dump.tex <==


\begin{table}[h!]
\scalebox{0.85}{
\begin{tabular}{@{}ccccccc@{}}
\cmidrule(l){2-7}
         & Baseline & BadNet & Blend & SIG   & WaNet & FTrojan \\ \midrule
CDA (\%) & 81.41   & 82.97  & 82.12 & 82.84 & 82.38 & 82.45   \\
ASR (\%) & -        & 99.09  & 97.54 & 99.87 & 99.09 & 97.86   \\ \bottomrule
\end{tabular}}
\caption{\textbf{2D Backdoor Attacks (Kinetics Sound).} Extending 2D backdoor attacks along the temporal dimension by simply repeating the attack on each frame achieves very high attack success rate while preserving or even improving clean data accuracy.}
\end{table}


\begin{table}[h!]
\scalebox{0.85}{
\begin{tabular}{@{}ccccccc@{}}
\cmidrule(l){2-7}
         & Baseline & BadNet & Blend & SIG   & WaNet & FTrojan \\ \midrule
CDA (\%) & 81.41    & 82.25  & 81.67 & 82.84  & 82.25 & 82.25   \\
ASR (\%) & -        & 99.74  & 95.79 & 100.00 & 99.61 & 95.27   \\ \bottomrule
\end{tabular}}
\caption{\textbf{2D Backdoor Attacks (Kinetics Sound).} Extending 2D backdoor attacks along the temporal dimension by applying the attacks on each frame with different parameters achieves a very high attack success rate while preserving or even improving clean data accuracy.}
\end{table}




\begin{table}[h!]
\scalebox{0.85}{
\begin{tabular}{@{}ccccccc@{}}
\cmidrule(l){2-7}
         & Baseline & BadNet & Blend & SIG   & WaNet & FTrojan \\ \midrule
CDA (\%) &  93.95  & 93.95 & 94.29 & 93.97 & 94.05 &  94.16  \\
ASR (\%) & -        & 99.63   & 99.26 & 99.97 & 99.84 & 99.34   \\ \bottomrule
\end{tabular}}
\caption{\textbf{2D Backdoor Attacks (UCF101).} Extending 2D backdoor attacks along the temporal dimension by simply repeating the attack on each frame achieves very high attack success rate while preserving or even improving clean data accuracy.}
\end{table}




\begin{table}[h!]
\scalebox{0.85}{
\begin{tabular}{@{}ccccccc@{}}
\cmidrule(l){2-7}
         & Baseline & BadNet & Blend & SIG   & WaNet & FTrojan \\ \midrule
CDA (\%) &  93.95  & 94.11   & 94.21 &  94.24 & 94.29 & 94.16   \\
ASR (\%) & -  & 99.97  & 99.44 & 100.00 & 99.79 &  99.34  \\ \bottomrule
\end{tabular}}
\caption{\textbf{2D Backdoor Attacks (UCF101).} Extending 2D backdoor attacks along the temporal dimension by applying the attacks on each frame with different parameters achieves a very high attack success rate while preserving or even improving clean data accuracy.}
\end{table}




\begin{table}[h!]
\scalebox{0.85}{
\begin{tabular}{@{}cccc@{}}
\cmidrule(l){2-4}
         & Frame Lag & Motion Blur & Frame Glitch  \\ \midrule
CDA (\%) &   &  &     \\
ASR (\%) &   &  & \\ \bottomrule
\end{tabular}}
\caption{\textbf{2D Backdoor Attacks (KineticsSound).} Extending 2D backdoor attacks along the temporal dimension by applying the attacks on each frame with different parameters achieves a very high attack success rate while preserving or even improving clean data accuracy.}
\end{table}


\begin{table}[h!]
\scalebox{0.85}{
\begin{tabular}{@{}cccc@{}}
\cmidrule(l){2-4}
         & Frame Lag & Motion Blur & Frame Glitch  \\ \midrule
CDA (\%) &   &  &     \\
ASR (\%) &   &  & \\ \bottomrule
\end{tabular}}
\caption{\textbf{2D Backdoor Attacks (UCF101).} Extending 2D backdoor attacks along the temporal dimension by applying the attacks on each frame with different parameters achieves a very high attack success rate while preserving or even improving clean data accuracy.}
\end{table}
